Millimeter Wave Line-of-Sight Blockage Analysis

Millimeter wave (mmWave) communication systems can provide high data rates but the system performance may degrade significantly due to mobile blockers and the user's own body. A high frequency of interruptions and long duration of blockage may degrade the quality of experience. For example, delays of more than about 10ms cause nausea to VR viewers. Macro-diversity of base stations (BSs) has been considered a promising solution where the user equipment (UE) can handover to other available BSs, if the current serving BS gets blocked. However, an analytical model for the frequency and duration of dynamic blockage events in this setting is largely unknown. In this thesis, we consider an open park-like scenario and obtain closed-form expressions for the blockage probability, expected frequency and duration of blockage events using stochastic geometry. Our results indicate that the minimum density of BS that is required to satisfy the Quality of Service (QoS) requirements of AR/VR and other low latency applications is largely driven by blockage events rather than capacity requirements. Placing the BS at a greater height reduces the likelihood of blockage. We present a closed-form expression for the BS density-height trade-off that can be used for network planning.

==> Chapters/Chapter1.tex <==
% Chapter 1

\chapter{Introduction} % Main chapter title

\label{Chapter1} % For referencing the chapter elsewhere, use \ref{Chapter1} 

%----------------------------------------------------------------------------------------

% Define some commands to keep the formatting separated from the content 
\newcommand{\keyword}[1]{\textbf{#1}}
\newcommand{\tabhead}[1]{\textbf{#1}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\file}[1]{\texttt{\bfseries#1}}
\newcommand{\option}[1]{\texttt{\itshape#1}}

%----------------------------------------------------------------------------------------

\section{Motivation}
% Millimeter-wave (mmWave) communication systems can provide high data rates of an order of a few Gbps~\cite{CellularCap-Rap}, suitable for the  Quality of Service (QoS) requirements for Augmented Reality (AR), Virtual Reality (VR), and the tactile Internet. For these applications, a user-equipment (UE) requires the data rate in the range of 100 Mbps to a few Gbps and an end-to-end latency in the range of 1 ms to 10 ms~\cite{ATTARVR}. However, mmWave communication systems are quite vulnerable to blockages due to higher penetration losses and reduced diffraction~\cite{tedmmWaveWillWork,bai2015coverage}. Even the human body can reduce the signal strength by 20 dB~\cite{georgeFading}. Thus, a Line-of-sight (LOS) link is highly desirable for mmWave systems. Furthermore, a mobile blocker can block the LOS path between User Equipment (UE) and Base Station (BS) for approximately 500 ms~\cite{georgeFading}. The frequent blockages of mmWave LOS links and high blockage duration can be detrimental to the low and ultra-low latency applications. 


% One potential solution to blockages in the mmWave cellular network can be macro-diversity of BSs and coordinated multipoint (CoMP) techniques. These techniques have shown a significant reduction in interference and improvement in reliability, coverage, and capacity in the current Long Term Evolution-Advance (LTE-A) deployments and other communication networks~\cite{kim2011analysis}. Furthermore, Radio Access Networks (RANs) are moving towards the cloud-RAN architecture that implements macro-diversity and CoMP techniques by pooling a large number of BSs in a single centralized baseband unit (BBU)~\cite{IBMCloudRAN,chen2011c}. As a single centralized BBU handles multiples BSs, the handover and beam-steering time can be reduced significantly~\cite{cloudRAN}.  

% In order to provide seamless connectivity for low and ultra-low latency applications, the proposed 5G mmWave cellular architecture needs to consider key QoS defining parameters such as the probability of blockage events, the frequency of blockages, and the blockage duration. \textcolor{blue}{The 5GPP requires the cellular link reliability to be 99.999\% \cite{mohr20165g}}. \textcolor{red}{ (insert some requirements for AR/VR requirements and give a citation.)} In general, the service interruption due to blockage events can be alleviated by caching the downlink contents at the BSs or the network edge~\cite{bastug2017toward}. However, caching the content \textcolor{blue}{more than about 40ms} may degrade the UE performance and may cause nausea to the user particularly for AR applications~\cite{westphal2017challenges}. Therefore, it is important to study the blockage probability, blockage frequency, and blockage duration for satisfying the desired QoS requirements. 
% % and the optimal amount of caching needed.     

% % In this paper, we consider an open park scenario where every available BS in the vicinity of the UE are potential serving BSs to the UE. 
% % We consider a scenario where all the blockers in the system are mobile blockers. Although there are many

% This work presents a simplified blockage model for the LOS link using tools from the stochastic geometry. In particular, our contributions are as follow:
% \begin{enumerate}
% \item We consider mobile blockers and calculate the rate of blockage of LOS link as a function of blocker density and the link length.
% \item The blockage events formulate an alternating renewal process with the exponential durations of alternate blocked and unblocked periods. We propose a Markov model for the blockage of $N$ BSs and derive the state probabilities.
% \item We evaluate the expected frequency and the expected duration of the blockage of all $N$ BSs in the range of UE, where the expectation is taken over the distribution of the distances between the UE and BSs and the number of BSs within the range according to the PPP model.
% \item Finally, we showed that our theoretical results match with Monte-Carlo simulations. We presented a case study for the minimum required BS density for specific mission-critical services. \textcolor{blue}{We also analysed the trade-off between BS height and density for satisfying the QoS requirements.}
% \end{enumerate}

% The rest of the paper is organized as follows. The related work is presented in Section \ref{sec:related-work} and the system model is described in Section \ref{sec:system-model}. Section \ref{sec:generalized} presents a generalized blockage model considering both self-blockage and dynamic blockages. Section~\ref{sec:numResults} evaluates our theoretical results with MATLAB simulations using random way-point mobility model of blockers. Finally, Section \ref{sec:conclusion} concludes the paper.


%----------------------------------------------------------------------------------------

\section{Literature Review}


%----------------------------------------------------------------------------------------

% \section{Contribution}


%----------------------------------------------------------------------------------------


==> Other/ish.tex <==
Hi

==> Tables/T21.tex <==
\begin{table}[!htbp] \centering 
  \caption{Descriptive Statistics} 
  \label{tab:descriptives} 
\begin{tabular}{@{\extracolsep{5pt}} cccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Maturity (Months) & Mean & Std. dev. & Minimum & Maximum & $\hat{\rho}(4)$ & $\hat{\rho}(26)$ & $\hat{\rho}(52)$ \\ 
\hline \\[-1.8ex] 
$1$ & $62.370$ & $27.904$ & $18.330$ & $140.140$ & $0.979$ & $0.757$ & $0.618$ \\ 
$3$ & $62.802$ & $28.023$ & $18.880$ & $141.010$ & $0.981$ & $0.775$ & $0.647$ \\ 
$6$ & $62.937$ & $28.167$ & $19.430$ & $141.570$ & $0.982$ & $0.791$ & $0.677$ \\ 
$9$ & $62.830$ & $28.237$ & $19.700$ & $141.410$ & $0.983$ & $0.804$ & $0.698$ \\ 
$12$ & $62.650$ & $28.252$ & $19.890$ & $140.810$ & $0.984$ & $0.815$ & $0.715$ \\ 
$15$ & $62.432$ & $28.220$ & $19.550$ & $140.160$ & $0.985$ & $0.824$ & $0.727$ \\ 
$18$ & $62.214$ & $28.174$ & $19.130$ & $139.570$ & $0.985$ & $0.831$ & $0.736$ \\ 
$24$ & $61.842$ & $28.046$ & $18.710$ & $138.900$ & $0.986$ & $0.841$ & $0.750$ \\ 
$30$ & $61.572$ & $27.935$ & $18.390$ & $138.390$ & $0.987$ & $0.849$ & $0.759$ \\ 
$36$ & $61.381$ & $27.859$ & $18.150$ & $137.720$ & $0.987$ & $0.854$ & $0.765$ \\ 
$48$ & $61.218$ & $27.858$ & $17.770$ & $137.080$ & $0.987$ & $0.861$ & $0.773$ \\ 
$60$ & $61.250$ & $27.996$ & $17.610$ & $136.910$ & $0.988$ & $0.867$ & $0.780$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 
